Scalable Diverse Model Selection for Accessible Transfer Learning

With the preponderance of pretrained deep learning models available off-the-shelf from model banks today, finding the best weights to fine-tune to your use-case can be a daunting task. Several methods have recently been proposed to find good models for transfer learning, but they either don't scale well to large model banks or don't perform well on the diversity of off-the-shelf models. Ideally the question we want to answer is, "given some data and a source model, can you quickly predict the model's accuracy after fine-tuning?" In this paper, we formalize this setting as "Scalable Diverse Model Selection" and propose several benchmarks for evaluating on this task. We find that existing model selection and transferability estimation methods perform poorly here and analyze why this is the case. We then introduce simple techniques to improve the performance and speed of these algorithms. Finally, we iterate on existing methods to create PARC, which outperforms all other methods on diverse model selection. We have released the benchmarks and method code in hope to inspire future work in model selection for accessible transfer learning.

==> latex/figures/1_concept_figure.tex <==
\begin{figure}[t]
\begin{center}
    \includegraphics[width=0.96\linewidth]{latex/figures/images/concept.png}
\end{center}

\caption{\textbf{Scalable Diverse Model Selection.} In this paper, we consider the task of selecting source model from a large, diverse off-the-shelf pretrained model bank that transfers well to some given target data.}

\label{fig:concept}
\end{figure}

==> sections/z_checklist.tex <==
\newpage
\section*{Checklist}

\begin{enumerate}

\newcommand{\explain}[1]{\\\hphantom{----}> {#1}}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
    \explain{Limitations are discussed in Sec.~\ref{sec:experiments} and Sec.~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
    \explain{We address the fact that non-experts might rely too heavily on recommendations from these model selection algorithms in Sec.~\ref{sec:conclusion}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} \explain{Code will be released with the public release of this paper. Including the code in this submission would deanonymize the authors.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} \explain{See the implementation details section in Sec.~\ref{sec:benchmark}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} \explain{We report error bars across different random probe set samples in every experiment.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} \explain{See the implementation details section in Sec.~\ref{sec:benchmark}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} \explain{Licenses for each model used are available in the supplement.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} \explain{The benchmark created in Sec.~\ref{sec:benchmark} will be released alongside the code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{} \explain{All content used that we didn't create ourselves is publicly released.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} \explain{We only use publicly available curated datasets.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
